Bandit Learning with Delayed Impact of Actions

We consider a stochastic multi-armed bandit (MAB) problem with delayed impact of actions. In our setting, actions taken in the past impact the arm rewards in the subsequent future. This delayed impact of actions is prevalent in the real world. For example, the capability to pay back a loan for people in a certain social group might depend on historically how frequently that group has been approved loan applications. If banks keep rejecting loan applications to people in a disadvantaged group, it could create a feedback loop and further damage the chance of getting loans for people in that group. In this paper, we formulate this delayed and long-term impact of actions within the context of multi-armed bandits. We generalize the bandit setting to encode the dependency of this "bias" due to the action history during learning. The goal is to maximize the collected utilities over time while taking into account the dynamics created by the delayed impacts of historical actions. We propose an algorithm that achieves a regret of $\tilde{\mathcal{O}}(KT^{2/3})$ and show a matching regret lower bound of $\Omega(KT^{2/3})$, where $K$ is the number of arms and $T$ is the learning horizon. Our results complement the bandit literature by adding techniques to deal with actions with long-term impacts and have implications in designing fair algorithms.

==> 1_intro.tex <==
Algorithms have been increasingly involved in high-stakes decision making. 
Examples include 
approving/rejecting loan applications~\citep{fuster2018predictably,kleinberg2018discrimination}, 
deciding on employment and compensation~\citep{bartik2016credit,cowgill2009incentive}, 
% college admissions~\citep{abdulkadirouglu2005boston}, 
and recidivism and bail decisions~\citep{angwin2016machine}.
Automating these high-stakes decisions has raised ethical concerns on whether it amplifies the discrimination bias against protected classes~\citep{obermeyer2019dissecting,chouldechova2017fair}. 
There have also been growing efforts towards studying algorithmic approaches to mitigate these concerns.
Most of the above efforts have focused on static settings:
a utility-maximizing decision maker needs to ensure her actions satisfy some fairness criteria at the decision time, 
without considering the long-term impacts of actions.
However, in practice, these decisions may often have long-term impacts on the rewards and well-beings for the people involved.
%To name a few examples,
For example,

\squishlist
    \item A regional financial institute may decide on the fraction of loan applications from different social groups to approve. 
    These decisions could affect the development of these groups: 
    The capability of applicants from a group to pay back a loan might depend on the group's socio-economic status, 
    which is influenced by how frequently applications from this group have been approved~\citep{bartlett2018consumer,cowgill2019economics}.
    \item The police department may decide on the amount of patrol time or the probability of patrol in a neighborhood (primarily populated with a demographic group). 
    The likelihood to catch a crime in a neighborhood might depend on how frequent the police decides to patrol this area~\citep{goel2016precinct,gelman2007analysis}. 
    %\item A university may decide on the ratio of applications from different groups to admit (e.g., via affirmative action rules). 
    %How successful a candidate from a group will be after college (e.g., their value to employers) might again depend on the socio-economic status of the group, influenced by the education opportunities that have been given~\citep{coate1993will,kleinberg2018discrimination}.
\squishend

These observations raise the following concerns. % in algorithmic fairness. 
If being insensitive with the long-term impact of actions, 
the decision maker risks treating a historically disadvantaged group unfairly. 
Making things even worse, these unfair and oblivious decisions might reinforce existing biases and make it harder to observe the true potential of a disadvantaged group.
While being relatively under-explored (but important), 
several recent works have looked at the delayed impact of actions in algorithm design.
However, these studies have focused on understanding the impact in a one-step delay of actions~\citep{liu2018delayed, kannan2019downstream, heidari2019long}, or a sequential decision making setting without uncertainty~\citep{mouzannar2019fair, zhang2019group, hu2018short,liu2019disparate}.  

This work departs from the above line of efforts by studying the long-term impact of actions in sequential decision making under uncertainty.
We generalize the multi-armed bandit setting by introducing the \emph{impact functions} that encode the dependency of the ``bias'' due to the action history of the learning to the arm rewards.
Our goal is to learn to maximize the rewards obtained over time, in which the rewards' evolution could depend on the past actions. 
This history-dependency structure of observed rewards makes our problem substantially more challenging. 
In particular, we first show that applying standard bandit algorithms leads to linear regret, i.e., existing approaches will obtain low rewards with a biased learning process.
Nonetheless, under relatively mild %and benign 
conditions for this dependency dynamics, we are able to present an algorithm with theoretical guarantees, based on a phased-learning template which smoothes out the historical bias during learning.
We then show a matching lower regret bound 
to demonstrate the optimality of our algorithm. 
Finally, we conduct a series of simulations showing that our algorithms compare favorably to other state-of-the-art methods proposed in other application domains. 

%\wt{do we need to include a paragraph to emphasize our contributions?}
%\noindent
%\textbf{Our Contributions.}
\cj{hmm, the below subsection and the above paragraph seem to overlap a lot}
\subsection{Our Contributions} % CJ: quite hesitated about the right headings (or if we need headings at all)
Our results and contributions can be summarized as follows:
\squishlist
    \item We formulate 
    %(see Section~\ref{sec:setting} for precise mathematical formulation of the problem) 
    the bandit learning problem with delayed impacts of actions. 
    We show that applying standard bandit algorithms leads to linear regret, i.e., existing approaches will obtain low rewards with a biased learning process. 
    The formulation and the negative results for standard bandit algorithms are included Section~\ref{sec:setting}).
    \item To deal with historical bias, we start with a simplified setting, where the impact only depends on the action deployed at the the current time. 
    This problem (we refer to action-dependent bandits) can of independent of interest and serves the building block for our main problem (we refer to history-dependent bandits). 
    By using tools from the combinatorial bandits, we design an algorithm which achieves $\tilde{\cO}(KT^{2/3})$ (see Section~\ref{sec:action}). After establishing the results for action-dependent bandits, we then propose algorithm for history-dependent bandits based on a phased-learning template which is able to smooth out the historical bias during learning, and gives us a sublinear regret bound of $\tilde{\cO}(KT^{2/3})$ (see Section~\ref{sec:history}).
    \item We prove a matching lower regret bound of $\Omega(KT^{2/3})$ for both bandit settings, 
    which means our solutions are order optimal in terms of the time horizon $T$ and the number of arms $K$ (see Section~\ref{sec:lowerbound}). 
    \item  We also conduct a series of simulations to demonstrate that our proposed algorithm outperforms state-of-the-art methods in practice (see Section~\ref{sec_simu}).
\squishend
The related work is included in Section~\ref{sec:related}.
The missing proofs of our main results are carried out in Appendices.



% ------- From WWW submission --------
\ignore{
To capture the effects that motivated our study, 
in this paper, we explore a variant of bandit settings in which the arm reward is neither i.i.d. nor adversarial, but instead is influenced by the historically made actions by the learner.
%of an arm could be neither of the above, 
%but instead is influenced by the learner's history of actions. 
We start by addressing a simplified setting, \emph{bandits with action-dependent rewards}, 
in which the reward of each arm is influenced by the action taken by the learner at each particular round \footnote{This setting can also be viewed as a special case as the history dependence is only encoded in the most recent action.}.
%probability the learner plans to pull the arm. 
%This setting serves as an easier starting point and is interesting on its own. 
%For example, consider deploying a learning strategy in security games \cite{balcan2015commitment}. 
%At each time step, the learner commits to a strategy, 
%and the attacker responds to the learner's committed strategy and therefore influences the reward of the arm. 
%Moreover, 
%While interesting on its own (see discussion in Section~\ref{sec:discussion-action-dependent}), 
This setting is an easier starting point and serves as the building block for our history-dependent case.
In each round of this setting, the learner first commits and announces her strategy (a probability distribution over all possible arms), 
the reward distribution of each arm is influenced by this announced strategy, 
the learner then receives the reward associated with the arm pulled by the realized strategy. 
We first demonstrate that the optimal strategy in this setting could be a mixed strategy, 
and therefore the learner needs to search over a continuous space of actions (probability simplex). 
While naively applying standard bandit algorithms on the discretized search space would lead to a regret of $\tilde{\cO}(T^{K/(K+1)})$ for $K$ arms and $T$ time rounds, 
we propose a UCB-like algorithm that utilizes the problem structure and achieves a significantly improved regret of $\tilde{\cO}(KT^{2/3})$.\footnote{We use $\tilde{\cO}(\cdot)$ to suppress the dependency of logarithmic factors.} 
Furthermore, we show a matching lower regret bound of $\Omega(KT^{2/3})$. 

We then consider our main setting, \emph{bandits with history-dependent rewards}, 
in which the reward of each arm is a function of the learner's action history. 
In this setting, the reward distribution of an arm is influenced by the time-discounted empirical frequency for the arm being selected.\footnote{Our results apply to a more general family of impact functions. See discussion in Section~\ref{sec:history-discussion}.}
We provide a template that helps reduce this problem to the above action-dependent setting with phases. 
Our reduction is inspired by the intuition of ``affirmative action'', in which we need to observe an action long enough to know its true potential.
In each phase, we start with an approaching stage to smooth out the historical bias caused by past taken actions. 
In the second stage of each phase, we then explore the true payoff under a targeted selection strategy, 
using a stylized UCB algorithm similar to the one we developed for the first action-dependent setting. 
We provide a good news via showing a $\tilde{\cO}(KT^{2/3})$ regret bound is again achievable that matches the one in the action-dependent case and show a matching lower regret bound of $\Omega(KT^{2/3})$.

This paper contributes to the bandit literature by formulating the long-term impact of actions,
which have implications in designing algorithms that are fair to different groups where learning has to be done with embedded historical biases due to past actions.
We explore the algorithm design in this space and propose algorithms that achieve $\tilde{\cO}(KT^{2/3})$ regret for a general class of impact functions and prove a matching lower bound.

}


==> 3_1_bandit_fail_main.tex <==
In this section, we show that an online algorithm which ignores its action's impact would suffer
linear regret. 
We consider two general bandit algorithms: TS (Thompson Sampling) and a mean-converging family of algorithms (which includes UCB-like algorithms).
These are the two most popular and robust bandit algorithms that can be applied to a wide range of scenarios.
We prove the negative results respectively.
In particular, we construct problem instances that could result in linear regret if the deployed algorithm ignore the action's impact.
\begin{exmpl}\label{exmpl_2}
Considering the following Bernoulli bandit instance with two arms, indexed by arm 1 and arm 2, i.e., $K= 2$.
For any $\epsilon\in [0, 1/2)$, define the expected reward of each arm as follows:
\squishlist
\item arm 1: $\rewfn_1(p) = p/(1-\epsilon)\cdot\mathbbm{1}(p\leq 1-\epsilon) + (2- \epsilon - p)\cdot\mathbbm{1}_(p\geq 1- \epsilon), \quad \forall p \in [0,1]$ 
\item arm 2: $\rewfn_2(p) = p/(2\epsilon)\cdot\mathbbm{1}_(p\leq \epsilon) + (-\frac{1}{2}p + \frac{1}{2}(1+\epsilon))\cdot\mathbbm{1}_(p\geq \epsilon), \quad \forall p \in [0,1]$ 
\squishend
\end{exmpl}
It is easy to see that $\vp^* = \{1-\epsilon, \epsilon\}$ is the optimal strategy for the above bandit instance.

We first prove the negative result of Thompson Sampling using the above example.
The Thompson Sampling algorithm can be summarized as below. 
\begin{algorithm}
  \caption{Thompson Sampling for Bernoulli bandits}
\begin{algorithmic}[1]
  \STATE {$S_i=0, F_i=0$.}
\FOR{$t=1, 2, \ldots,$}
    \STATE For each arm $i=1,2$, sample $\theta_i(t)$ from the $\Beta(S_i+1, F_i+1)$ distribution. 
    \STATE Play arm $a_t := \arg \max_i \theta_i(t)$ and observe reward $\rewob_t$.
    \STATE If $\rewob_t=1$, then $S_{a_t}=S_{a_t}+1$, else $F_{a_t}=F_{a_t}+1$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{figure}[!htb]
  \center{\includegraphics[width=0.65\textwidth] {pics/bandit_fail_instance.pdf}}
  \caption{The expected reward defined in Example \ref{exmpl_2}: arm 1 (left) and arm 2 (right).}
  \label{fig:arm_reward_exml_2} 
\end{figure}

\begin{lemma}\label{lem:TS_fail}
For the reward structure defined in Example \ref{exmpl_2},
Thompson Sampling would suffer linear regret if it doesn't consider the action's impact it deploys at every time round, namely, it takes the sample mean as the true mean reward of each arm.
\end{lemma}

Before we proceed, we first prove the following strong law of large numbers in Beta distribution.
We note that the below two lemmas are not new results and can be found in many statistical books. 
We provide proofs here for the sake of making the current work self-contained.
% \input{auxiliary_lemma}

We now ready to prove Lemma~\ref{lem:TS_fail}.
\begin{proof}
We prove this by contradiction.
Let $\reg(T)$ denote the expected regret incurred by TS up to time round $T$, and $N_t(\vp) = \sum_{s =1}^t \mathbbm{1}_{\vp(s) = \vp}$ denote the number of rounds when the algorithm deploys the (mixed) strategy $\vp \in \Delta_K$.
Furthermore, let $S_i(t) (\text{resp. }F_i(t))$ denote the received $1_s(\text{resp. } 0_s)$ of arm $i$ up to time round $t$.
Recall that in Thompson Sampling, we have $\Psymb(a_t = 1) = \Psymb\big(\theta_1(t) > \theta_2(t)\big)$.
By the reward function defined in Example \ref{exmpl_2}, it's immediate to see that 
\begin{align*}
S_1(T) \geq (1-\epsilon)N_T(\vp^*); \quad F_1(T)\leq T - N_T(\vp^*); \quad S_2(T)\geq 0.5\epsilon N_T(\vp^*); \quad F_2(T)\geq 0.5\epsilon N_T(\vp^*).
\end{align*}
Now suppose Thompson Sampling achieves sublinear regret, i.e., $\reg(T) = o(T)$, which implies following
\begin{align*}
\lim_{T\rightarrow \infty} \frac{T - N_T(\vp^*)}{T} = 0.
\end{align*}
Thus, by the strong law of large numbers and invoking Lemma \ref{lem: beta_delta_approx}, the sample $\theta_1(T+1)\sim\Beta(S_1(T), F_1(T))$ and $\theta_2(T+1)\sim\Beta(S_2(T), F_2(T))$ will converge as follows:
\begin{align}
\lim_{T\rightarrow \infty} \theta_1(T+1)  = 1; \quad \lim_{T\rightarrow \infty} \theta_2(T+1)  = 0.5.
\end{align}
Then it's almost surely that $\lim_{T\rightarrow \infty} \Psymb(a_{T+1} = 1) = \lim_{T\rightarrow \infty}\Psymb\big(\theta_1(T+1) > \theta_2(T+1)\big) = 1$.
This leads to following holds for sure
\begin{align*}
S_1(s+1) = S_1(s) + 1, \forall s > T.
\end{align*}
Thus, consider the regret incurred from the $(T+1)-$th round to $(2T)-$th round, the regret will be 
\begin{align*}
\reg(2T)- \reg(T) = \sum_{s={T+1}}^{2T} U(\vp(s)) = 0.5T\epsilon,
\end{align*}
where the second equality follows that $ \vp(s) = (1, 0)$ holds almost surely from $T+1$ to $2T$.
This shows that $\lim_{T\rightarrow\infty} \frac{\Esymb[\reg(2T)]}{2T} = \epsilon/4$, which contradicts that the algorithm achieves the sublinear regret. 
\end{proof}

We now show that a general class of algorithms, which are based on \emph{mean-converging}, will suffer linear regret if it ignores the action's impact.
This family of algorithms includes UCB algorithm in classic MAB problems.
\begin{definition}[Mean-converging Algorithm~\citep{schmit2018human}]
Define $I_k(t) = \{s: a_s = k, s < t\}$ as the set of time rounds such the arm $k$ is chosen.
Let $\bar{\rewfn}_k(t) = \frac{1}{|I_k(t)|} \sum_{s\in I_k(t)} \rewob_s$ be the empirical mean of arm $k$ up to time $t$.
The mean-converging algorithm $\cA$ assigns $s_k(t)$ for each arm $k$ if following holds true:
\squishlist
\item $s_k(t)$ is the function of $\{\rewob_s: s\in I_k(t)\}$ and time $t$;
\item $\Psymb(s_k(t) = \bar{r}_k(t)) = 1$ ~~ if ~~$\liminf_{t}\frac{|I_k(t)|}{t} > 0$.
\squishend
\end{definition}
\begin{lemma}
For the reward structure defined in Example \ref{exmpl_2},
the mean-converging Algorithm will suffer linear regret if it mistakenly take the sample mean as the true mean reward of each arm.
\end{lemma}
\begin{proof}
We prove above lemma by contradiction.
Let $N^\cA_t(\vp)$ denote the number of plays with deploying the strategy $\vp$ by algorithm $\cA$ till time $t$.
Suppose a mean-converging Algorithm $\cA$ achieves sublinear regret, then it must have $\lim_{T\rightarrow \infty} {N^\cA_T(\vp^*)}/{T} > 0$ and $\lim_{T\rightarrow \infty} \big({T - N^\cA_T(\vp^*)}\big)/{T} = o(T)$. 
By the definition of mean-converging algorithm and recall the reward structure defined in Example \ref{exmpl_2}, the score $s_T(1)$ assigned to arm 1 by the algorithm $\cA$ must be converging to 1, and the score of $s_T(2)$ assigned to arm 2 must be converging to 0.5.
By the strong law of large numbers, it suffices to show that $\Psymb(\vp(t) = \{1,0\}) = 1. \forall t\geq T+1$, which implies the algorithm $\cA$ would suffer linear regret after $T$ time rounds and thus completes the proof.
\end{proof}


==> 7_1_figures.tex <==
\begin{figure*}[th]
   \centering
   \subfigure[Action-dependent]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_1_cumuReg_new.pdf}
      \label{fig_1}
   }
   \subfigure[$\gamma = 0.2$]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_2_cumuReg_gamma_2_new.pdf}
      \label{fig:weak-correlation}
   }
   \subfigure[$\gamma = 0.4$]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_2_cumuReg_gamma_4_new.pdf}
      \label{fig:gamma_0.2}
   }
  \subfigure[$\gamma = 0.6$]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_2_cumuReg_gamma_6_new.pdf}
      \label{fig:gamma_0.6}
   }
  %\vspace{-5pt}
  \caption{(a): \textmd{Behavior of the different algorithms for \action.} (b)-(d): \textmd{Behavior of the different algorithms for \history~on different $\gamma$.}}
  \vspace{-12pt}
  \label{fig:main}
\end{figure*}


\begin{figure*}[th]
   \centering
   \subfigure[$K = 3$]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_3_cumuReg_K_3_new.pdf}
      \label{fig:K_3}
   }
   \subfigure[$K = 4$]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_3_cumuReg_K_4_new.pdf}
      \label{fig:K_4}
   }
   \subfigure[$K = 5$]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/fig_3_cumuReg_K_5_new.pdf}
      \label{fig:K_5}
   }
  \subfigure[different ratio]{
   	\includegraphics[width=0.45\columnwidth, keepaspectratio]{pics/different_ratio_new.pdf}
      \label{fig:ratio}
   }
    %\vspace{-5pt}
    \caption{(a)-(c): \textmd{Behavior of the different algorithms on different $K$, the remaining parameters are the same with the simulations in comparison on different $K$.} (d): \textmd{The performance of our algorithms on different ratios, we set $K=2$ and remaining parameters are also same as before.}}
    \vspace{-12pt}
    \label{fig:K_and_ratio}
\end{figure*}


==> exp.tex <==
We have performed synthetic experiments to empirically evaluate the performance of our proposed solution with a set of baselines.
%state-of-the-art bandit algorithm baselines.

\subsection{Evaluations for \action}
We first evaluate our proposed algorithm on \action~against the following state-of-the-art bandit algorithms.
\squishlist
\item \textbf{EXP3}:
One natural baseline is applying EXP3 \citep{auer2002nonstochastic} on the space of base arms.
While EXP3 is designed for adversarial rewards, it is competing with the best fixed arm in hindsight and might not work well in our setting since the optimal strategy is randomized.

\item \textbf{EXP3-Meta-Arm (mEXP3)}: 
To make a potentially more fair comparison, we also implement EXP3 on the meta-arm space. 
We denote it as mEXP3 in the following discussion.
\item \textbf{CUCB} \citep{chen2016combinatorial,wang2017improving}:
This algorithm is designed to solve combinatorial semi-bandit problem, 
which chooses $m$ arms out of $M$ arms at each round and receives only the rewards of selected arms. 
Mapping to our setting, $M = K / \epsilon$ represents the total number of discretized arms, 
$m=K$ is the number of base arms, and the selection of $m$ arms is constrained to satisfy the probability simplex constraint.
\squishend
In the simulations, we set $K = 2$ for simplicity.
Moreover, $\rewfn_k(p_k)$ is chosen such that $\rewfn_k(p_k)$ is maximized when $0<p_k<1$. 
In particular, we define $\rewfn_k(p_k)$ as
a scaled Gaussian function : $\rewfn_k(p_k) = f(p_k|\tau_k, 0.5)/C_k$, where $f(x|\tau, \sigma^2)$ is the pdf of Gaussian distribution with the mean $\tau$ and variance $\sigma^2$, and $C_k = f(\tau_k|\tau_k, \sigma^2)$ is a constant ensuring $\rewfn_k(p_k) \in [0,1], \forall p_k\in[0,1]$. 
For each arm $k$, $\tau_k$ is uniformly draw from 0.45 to 0.55 and the instantaneous reward is drawn from a Bernoulli distribution with the mean of $\rewfn_k(p_k(t))$, i.e., $\rewob_t(p_k(t)) \sim \Ber(\rewfn_k(p_k(t)))$.
And the ratio $\rho$ is set to 0.2.
For each algorithm we perform 40 runs for each of independent 40 values of the corresponding parameter, and we report the averaged results of these independent runs, where the error bars correspond to $\pm2$ standard deviations.

%The results of the experiment are displayed in Figure \ref{fig_1}, where we plot the cumulative regret against the number of rounds $T$. 
% All algorithms have a single parameter that governs the degree of exploration. 
%The experimental results show that compared with EXP3, mEXP3 and CUCB, Algorithm \ref{algo:action_UCB} can significantly reduce the cumulative regret by exploiting specific reward structure.
The results, shown in Figure~\ref{fig_1}, demonstrate that our algorithm significantly outperforms the baselines.
As expected, mEXP3 works better than EXP3 algorithm when $T$ is large, since the former searches the optimal strategies in the meta arm space. 
Our algorithm outperforms mEXP3 and CUCB since we utilize the problem structure, which reduces the amount of explorations.

\subsection{Evaluations for \history}
We now evaluate our proposed algorithm for \history~via comparing against the following baselines from non-stationary bandits.
Note that, while CUCB performs reasonably well in action-dependent case, it does not apply in history-dependent case, since we cannot \emph{select} the time-discounted frequency (which maps to the arm in CUCB) as required in CUCB.
\squishlist

\item \textbf{Discounted UCB} \citep{garivier2011upper,kocsis2006discounted}:
Discounted UCB (DUCB) is an adaptation of the standard UCB policies that relies on a discount factor $\gamma_\DUCB \in (0,1)$.
This method constructs an $\UCB: \bar{\rewfn}_{t}(k, \gamma_\DUCB) + c_t(k,\gamma_\DUCB)$ for the instantaneous expected reward, 
where the confidence is defined as $c_t(k, \gamma_\DUCB) = 2\sqrt{\frac{\xi \ln(n_t)}{N_t(k, \gamma_\DUCB)}}$, for an appropriate parameter $\xi$, 
% $n_t = \sum_{k=1}^K N_t(k, \gamma_\DUCB)$, 
$N_t(k, \gamma_\DUCB) = \sum_{s=1}^t\gamma_\DUCB^{t-s} \mathbbm{1}_{(a_s = k)}$,
and the discounted empirical average is given by
$\bar{\rewfn}_{t}(k, \gamma_\DUCB) = \frac{1}{N_t(k, \gamma_\DUCB)} \cdot\sum_{s =1}^t\gamma_\DUCB^{t-s} \rewob_{s}(k)\mathbbm{1}_{(a_s = k)}$.

\item \textbf{Sliding-Window UCB} \citep{garivier2011upper}:
Sliding-Window UCB (SWUCB) is a modification of DUCB, instead of averaging the rewards over all past with a discount factor, SWUCB relies on a local empirical average of the observed rewards, for example, using only the $\tau$ last plays.
Specifically, this method also constructs an $\UCB: \overbar{\rewfn}_{t}(k, \tau) + c_t(k,\tau)$ for the instantaneous expected reward. 
The local empirical average is given by
$\overbar{\rewfn}_{t}(k, \tau) = \frac{1}{N_t(k, \tau)}\sum_{s =t-\tau+1}^t \rewob_{s}(k)\mathbbm{1}_{(a_s = k)}$, $N_t(k, \tau) = \sum_{s =t-\tau+1}^t\gamma_\DUCB^{t-s} \mathbbm{1}_{(a_s = k)}$ and the confidence interval is defined as $c_t(k, \gamma_\DUCB) = 2\sqrt{\frac{\xi \ln(\min(t, \tau))}{N_t(k, \tau)}}$.
\squishend
We use \emph{grid searches} to determine the algorithms' parameters.
For example, in DUCB, the discount factor was chosen from $\gamma_\DUCB\in\{0.5, 0.6, \ldots 0.9\}$, while the window size of SWUCB was chosen from $\tau\in\{10^2,\ldots, 5\times 10^2\}$.
Besides above algorithms, we also implement the celebrated non-stationary bandit algorithm EXP3.

We chose $K$ and $\rewfn_k(p_k)$ to be the same as the experiments in action-dependent case.
And the discount factor is chosen as $\gamma_\DUCB = 0.8$ and the window size for SWUCB is chosen as 200 via the grid search, and $\xi$ is set to 1.
We examine the algorithm performances under different $\gamma$ (the parameter in time-discounted frequency), 
with smaller $\gamma$ indicating that arm rewards are more influenced by recent actions. 
As seen in Figures~\ref{fig:gamma_0.2}-\ref{fig:gamma_0.6}, our algorithm outperforms all baselines in all $\gamma$ but the improvement is more significant with small $\gamma$.
This is possibly due to that most non-stationary bandit algorithms have been focusing on settings in which the change of arm rewards over time is not dramatic. 



We also examine our algorithm with larger number of base arms $K$ with comparing to above baseline algorithms and the performance of our algorithm on different ratios $\rho$. 
The results are presented in Figure~\ref{fig:K_and_ratio}
and show that our algorithm consistently performs better than other baselines when $K$ goes large.
The results also suggest that our algorithm is not sensitive to different $\rho$, though one could see the regret is slightly lower when $\rho$ is increasing, which is expected from our regret bound.




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> missing_exps.tex <==
% We provide the simulations on the comparisons of our algorithms with other baseline algorithms on different $K$, and the performance of our algorithms on different ratios. 
% The results are presented in Figure~\ref{fig:K_and_ratio}.

\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/fig_3_cumuReg_K_3.pdf}
        \caption{$K = 3$}   
        \label{fig:K_3}
    \end{subfigure}
        % \hfill
    \begin{subfigure}[b]{0.40\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{pics/fig_3_cumuReg_K_4.pdf}
    	\caption{$K = 4$}
    	\label{fig:K_4}
    \end{subfigure}
        \vskip\baselineskip
    \begin{subfigure}[b]{0.40\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{pics/fig_3_cumuReg_K_5.pdf}
    	\caption{$K = 5$}
    	\label{fig:K_5}
    \end{subfigure}
    	\quad
    \begin{subfigure}[b]{0.40\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{pics/different_ratio.pdf}
        \caption{different ratio}
        \label{fig:ratio}
    \end{subfigure}
    \caption{(a)-(c): \textmd{Behavior of the different algorithms on different $K$, the remaining parameters are the same with the simulations in comparison on different $K$.} (d): \textmd{The performance of our algorithms on different ratios, we set $K=2$ and remaining parameters are also same as before.}}
    \label{fig:K_and_ratio}
\end{figure*}
